Low-bit Quantization for Deep Graph Neural Networks with Smoothness-aware Message Propagation

Graph Neural Network (GNN) training and inference involve significant challenges of scalability with respect to both model sizes and number of layers, resulting in degradation of efficiency and accuracy for large and deep GNNs. We present an end-to-end solution that aims to address these challenges for efficient GNNs in resource constrained environments while avoiding the oversmoothing problem in deep GNNs. We introduce a quantization based approach for all stages of GNNs, from message passing in training to node classification, compressing the model and enabling efficient processing. The proposed GNN quantizer learns quantization ranges and reduces the model size with comparable accuracy even under low-bit quantization. To scale with the number of layers, we devise a message propagation mechanism in training that controls layer-wise changes of similarities between neighboring nodes. This objective is incorporated into a Lagrangian function with constraints and a differential multiplier method is utilized to iteratively find optimal embeddings. This mitigates oversmoothing and suppresses the quantization error to a bound. Significant improvements are demonstrated over state-of-the-art quantization methods and deep GNN approaches in both full-precision and quantized models. The proposed quantizer demonstrates superior performance in INT2 configurations across all stages of GNN, achieving a notable level of accuracy. In contrast, existing quantization approaches fail to generate satisfactory accuracy levels. Finally, the inference with INT2 and INT4 representations exhibits a speedup of 5.11 $\times$ and 4.70 $\times$ compared to full precision counterparts, respectively.

==> algorithm/kmeans_quant_criteria.tex <==
\begin{algorithm}[tb]
	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
	\renewcommand{\algorithmicensure}{\textbf{Output:}}
	\caption{Node-wise Quantization}%{Partition-based Index}
	\label{alg:node-wise quantization}
	\begin{algorithmic}[1]
		\REQUIRE $T$, $b$, $\tau$, $\tau_{1}$, $\tau_{2}$, $k$ 
		\ENSURE  $B$
		 	\STATE $B$$\leftarrow$Initialize $2^{b}$ centroids with equal-width bins,  $I_{B}$$\leftarrow$the reconstruction point index for $T$,   and $B^{pre}=\{\}$  
		       \FOR{$i$ in $\{ 1,2,...,d\}$}
		       \WHILE{$\|B - B^{pre}\|_{2} > \tau$}
		       \STATE $B^{pre}=B$  
		       \FOR{$j$ in $\{ 1,2,...,m\}$}
		    \STATE $B$, $I_{B}$$\leftarrow$$intraclass\_update$($T$, $B$, $I_{B}$, $j$, $i$, $\tau_{1}$, $k$)
		    \IF{$j > 1$}
		    \STATE $B$, $I_{B}$$\leftarrow$$interclass\_update$($T$, $B$, $I_{B}$, $j$, $i$, $\tau_{2}$, $k$)
		    \ENDIF
		        \ENDWHILE
		   \ENDFOR 
		\ENDFOR   
	%	\STATE break;

	    \STATE \textbf{return}  $B$
	\end{algorithmic}  
\end{algorithm}


\begin{algorithm}[tb]  
\renewcommand{\thealgorithm}{}
\floatname{algorithm}{Function}
\setcounter{algorithm}{0}
  	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
	\renewcommand{\algorithmicensure}{\textbf{Output:}}
	\caption{$intraclass\_update$($T$, $B$, $I_{B}$, $j$, $i$, $\tau_{1}$, $k$)}
	\label{alg:intraclass_update}
	\begin{algorithmic}[1]
	%	\REQUIRE the grid region $\{S_{g_s,i}\}$, $Cq$
		\ENSURE $B$, $I_{B}$. 
		\STATE min\_v, max\_v $\leftarrow$ $T_{j,i}$, [b_s, b_e] $\leftarrow$ [min\_v, max\_v]
% 		\STATE if {($b_s-k$)$\leq$0}  {$b_s=1$} else  {$b_s$=$b_s-k$}
% 		\STATE if {($b_e+k$)$>$|B|}  {$b_e=|B|$} else  {$b_e$=$b_e+k$}
% 		\IF{($b_s-k$)$<$0}{$b_s=0$} \ELSE{$b_s$=$b_s-k$}\ENDIF
		% \IF{all ($s_{i,x}, s_{i,y} = 1\&$ no padding) or $s_{i,x}, s_{i,y}$ = 0}
		  %      \STATE return
		 %\ELSE
		   %\STATE   $Cq.append(\{S_{g_s,i}\})$.
		  \FOR{$t$ in $[b_s,b_e]$}
		  %  \STATE $temp$ = $\{\}$
		   \FOR{$p$ in $[-k,k]$}
		   \IF{$t+p< b_s$ or $t+p> b_e$ or $p==0$}
		      \STATE continue      
		   \ENDIF
		  % \STATE $temp$ = $temp.append(T_{j,i}[t+p])$
		   \STATE $temp_s$ = $(T_{j,i}[t+p] \cup T[t]).mean()$
		            \IF{$\|temp_s - B[t]\|_{2}>\tau_{1}$ and $p > 0$}
		                   \STATE break
		             \ELSE 
		               $B[t]=temp_s$, update $I_{B}$
		             \ENDIF
         
    		        \ENDFOR
		  \ENDFOR
		   \STATE \textbf{return}  $B$, $I_{B}$
	\end{algorithmic}  
\end{algorithm}


\begin{algorithm}[tb]  
\renewcommand{\thealgorithm}{}
\floatname{algorithm}{Function}
\setcounter{algorithm}{0}
  	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
	\renewcommand{\algorithmicensure}{\textbf{Output:}}
	\caption{$interclass\_update$($T$, $B$, $I_{B}$, $j$, $i$, $\tau_{2}$, $k$)}
	\label{alg:interclass_update}
	\begin{algorithmic}[1]
	%	\REQUIRE the grid region $\{S_{g_s,i}\}$, $Cq$
		\ENSURE  $B$, $I_{B}$. 
		\STATE $\{b_{p}\}$ $\leftarrow$ $I_{B}[j,i]$.unique()
		% \IF{all ($s_{i,x}, s_{i,y} = 1\&$ no padding) or $s_{i,x}, s_{i,y}$ = 0}
	        \FOR{$t$ in $\{b_{p}\}$}
	        \STATE $class\_num$ = $T_{\cdot,i}[t]$.class()
	        \IF{$class\_num==1$}
		         continue
		    \ELSE 
		  %  \STATE $temp$ = $T_{j,i}[t]$
		         \FOR{$l$ in $[-k,k]$}
		          \IF{$t+l\leq 0$ or $t+l>|B|$ or $l==0$}
		      \STATE continue      
		   \ENDIF
		     \STATE $temp_s$ = $(T_{j,i}[t] \cup T[t+l]).mean()$
		            \IF{$\|temp_s - B[t]\|_{2}>\tau_{2}$}
		                   \STATE break
		             \ELSIF{$(temp \cup T_{\cdot,i}[t+l]).class()<class\_num$}
		               $B[t]=temp_s$, update $I_{B}$
		             \ENDIF
		    
		  %  \IF{$(temp \cup T[t]).class()<class\_num$}
		    
		    
		    
		  %  \ENDIF
		    \ENDFOR
		    \ENDIF
		    
		    \ENDFOR
		    \STATE \textbf{return}  $B$, $I_{B}$
	\end{algorithmic}  
\end{algorithm}

\textbf{Algorithm Explanation}
Motivation: The QAT (Quantization-aware training) for neural network usually can reduce the accuracy deteriorates by making the quantization loss aware at neural network training, even at extremely low-precision (e.g., 2-bit) \cite{choi2019accurate}.
The existing work reduced the MSE (mean sauqred errors) by clipping the quantization range \cite{choi2019accurate} and learning the dynamic resolution \cite{zhaoyang2021differentiable}, which depends on the learnable differentiable parameters. However, there are some different challenges for GNN quantization. 
First, there are multiple cascading quantization elements in each layer, e.g., inputs to each layer, message propagating between nodes, the inputs and outputs at aggregation stage as well as the outputs of the update stage \cite{tailor2020degree}. A large loss on one element will accumulate on these cascading elements leading to accuracy deterioration. Second, training the quantized models can be highly unstable \cite{tailor2020degree}, and in our experimental study, by applying dynamic quantization range for GNN which has been proven to be powerful for CNN quantization, we can achieve almost full-precision accuracy with 4-bit quantization at the best case, but the performance is still unstable even though the quantization loss can be always at lower values. Third, the existing dynamic resolution quantization for CNN \cite{zhaoyang2021differentiable} aims to reduce the quantization loss overall, however, the quantized element in GNN corresponds to nodes from different classes, the small quantization loss does not necessarily guarantee classification accuracy which reflect the node-level similarity.

To achieve robust GNN quantization, we design the node-wise quantization method to reduce the intra-class distance and increase the inter-class distance, which can be applied for every quantizable element mentioned above.
The process of node-wise quantization is described as \textbf{Algorithm \ref{alg:node-wise quantization}}. In Line 1, given b-bit, the $2^{b}$-length centroids $B$ is initialized with the midpoints of the equal-length bin. Line 3--Lin 8 iteratively collect the $i$-dimension values of the same class to the smaller number of bins ($intraclass\_update$ in Line 6), and distribute the values from $m$ different classes to different bins ($interclass\_update$ in Line 8), which need to satisfy the given distortion tolerances $\tau_{1}$ and $\tau_{2}$, respectively. In \textbf{Function $intraclass\_update$}, $T_{j,i}$ represents the set for the $j$-th class at the $i$-th dimension. In Line $1$, $b_s$ and $b_e$ represents the range of the bins that can cover $T_{j,i}$.
$temp$ = $T_{j,i}[t]$ in Line 3 denotes the subset of $T_{j,i}$ that is assigned to the $t$-th bin. 
From Line 4--11, we iteratively check if $T_{j,i}[t]$ can be assigned to the neighbour bin (t+p), while guaranteeing the deviation between the current centroid ($B[t]$) and the potential centroid ($temp_s$) will not exceed the given distortion threshold $\tau_{1}$ (Line 9). At Line 1 of \textbf{Function $interclass\_update$}, $I_{B}[j,i]$ denotes the bin index for the $j$-th class nodes at the $i$-th dimension, $\{b_{p}\}$ denotes the bins that $T_{j,i}$ is indexed.
$T_{\cdot,i}[t]$.class() in Line 3 represents the number of classes that are indexed by the $t$-th bin at the $i$-th dimension. Line 7--13 assign $T_{j,i}[t]$ to the neighbor bin ($t+l$) if the deviation will not exceed the given threshold $\tau_{2}$ and the number of classes assigned to the new bin is smaller than $class\_num$, which aims to distribute different classes to diverse bins.

==> plots/2-quantization_basics.tex <==
%\section{GNN Quantization}
\section{Background and Analysis}
This section provides an introduction to GNNs and quantization, analysis of the quantization errors and the oversmoothing issue in GNNs, providing technical motivation and insights for the developed methods. 
% \section{Grouping Quantization for GNN }
%In this section, we describe the distribution of multiple tensor-valued elements and design grouped quantization over multiple tensors. 
% \TG{What is the goal of this section? To me it looks like background and identifying the challenged with GNN quantization}
\subsection{Preliminaries}
A graph $\mathcal{G}$ is represented as $\mathcal{G} = (V, E, \mathbf{X})$, where $V = \{v_1, v_2 \cdots v_n\}$ is the set of $n$ nodes $|V|=n$, $E$ is the set of all edges, $\mathbf{H^l}$ = $[\mathbf{h}^l_{1}, \mathbf{h}^l_{2}, \cdots \mathbf{h}^l_{n}]^{\top}$ is the node feature (embedding) matrix for  layer $l \in K$ where $K$ represents the number of layers in $\mathcal{G}$, and $\mathbf{h}_{i} \in \mathbb{R}^{d_{l}}$ is the feature vector for $v_i\in V$ node with initial $\mathbf{H^0}=\mathbf{X}$.  The adjacency matrix of $\mathcal{G}$ is a binary matrix $\mathbf{A} \in \mathbb{R}^{n \times n}$, where $\mathbf{A}(i,j)=1$ if the edge between  nodes $v_i$ and $v_j$ exists ($e_{ij} \in E$), and $0$ otherwise.

Popular GNN architectures are an extension of the CNN architectures modified to handle graph data. 
%in which neighborhood definition is not trivial as in the case of image etc. 
These GNNs consist of sequence of layers with three main functions for each layer: message passing, aggregation and update. This framework is generally called Message Passing NNs (MPNN) \cite{Gilmer2017MPNN}. Each message, which is a flow of data from node's neighbors is aggregated and joined with existing embedding to form the new embedding for the respective node as given in Equation~\ref{eq:MPNN} where $\mathcal{N}_u$ is the neighbor nodes of node $u$. Feed-forward iteration starts with the initial embeddings, $\mathbf{h}^0_u = \mathbf{x}_{u}$.
\begin{equation}
\mathbf{h}^{(l+1)}_{u} ={Update}_l(\mathbf{h}^l_u,Aggregate_l({\mathbf{h}_v^l, \forall v \in \mathcal{N}_u})
\label{eq:MPNN}
\end{equation}

There are different aggregation and update functions proposed for various architectures \cite{TNNLS2021GNNSurvey}. We consider the popular GCN (Graph Convolutional Network) architecture and update function provided in Equation~\ref{eq:GCN} with an activation function $\sigma$ and learnable weight matrix $\mathbf{W_l}$\cite{kipf2017GCN}.
\begin{equation}
\mathbf{h}_{(l+1)}^{u} =\sigma \bigg( \sum_{v \in \mathcal{N}^u \cup u}\frac{1}{\sqrt{d_u d_v}}\mathbf{W}_l\mathbf{h}_{l}^{v}) \bigg)
\label{eq:GCN}
\end{equation}
Time complexity of GCN is $O(L ||A||_0 d + Lnd^2)$ and memory complexity $O(Lnd + Ld^2)$ where $L$ is the number of layers, $||A||_0$ is the number of non-zeros entries in $\mathbf{A}$ \cite{ClusterGCN2019}. 
% These figures illustrate the increase in computational load for increasing scale of graphs and feature dimensions emphasising the importance of decreasing the computational and memory load with quantization methods. 

\citet{ma2021unified} unify the representative GNN models, such as GCN, GAT, PPNP, and APPNP by considering them as solving the graph denoising problem.
\begin{equation}
\centering
\begin{aligned}
% \left
% &\underset{S_{l}, F}{\text{min}} \quad \mu_{1}
&\underset{\mathbf{H}}{\text{argmin}} \quad \frac{1}{2}\|{\mathbf{H-X}}\|_{F}^{2} + \frac{\mu}{2} \mathbf{tr(H^{\top}LH)} 
% , l = 0,1,..., L
\end{aligned}
\label{eq:basic_denoising}
\end{equation}
where $\mathbf{H}$=$[\mathbf{h}_{1}, \mathbf{h}_{2}, \cdots \mathbf{h}_{n}]^{\top}\in \mathbb{R}^{n\times d}, \mathbf{L}\in \mathbb{R}^{n\times n}$ represents the graph Laplacian matrix. The first term enforces the embeddings $\mathbf{H}$ to be close to the graph input feature matrix $\mathbf{X}$,  the second term imposes the global smoothness by enforcing similarity in the connecting nodes. Specifically,
\begin{equation}
\mathbf{tr(H^{\top}LH)} =\sum_{(v_{i},v_{j}) \in E}\| {\mathbf{h}_{i}} - {\mathbf{h}_{j}}\|_{2}^{2}
\label{eq:edgedifference}
\end{equation}
Recently $\ell_{1}$ based constraints are also used as an alternative local smoothness criteria with \textbf{EMP} (Elastic Message Passing) \cite{liu2021elastic}. 


%where $\Delta$ is the quantization step.  
%For simplicity, $Q(U, s, z)$ and $D(U_q, s, z)$ are represented as $Q(U)$ and $D(U_q)$ respectively in the following content. The de-quantization value is represented as $\hat{U}$=$D(U_q, s, z)$.

% if the density distribution at $\Delta$ cannot be accurately approximated by a linear function.
% Some existing work approximates the density function $f(\cdot)$ as a linear function at each quantization step, then the granular distortion depends on the size of $\Delta$ and if the values are linearly distributed. 

\subsection{GNN Quantization}\label{gnn_quantization_introduction}
There are major challenges in designing an effective quantization solution tailored for GNNs. GNNs involve more types of elements to be quantized compared to conventional CNNs.
The values to be quantized in GNNs include the inputs of each layer ($\mathbf{h_l}$), the weights ($\mathbf{W_l}$), the message between nodes, the inputs and outputs of the aggregation stage and the output of the update stage. This is in contrast to quantizing only weights and activations in CNNs. Ineffective quantization for any element in GNNs will increase the distortions of the later message propagation process. Moreover, as the variance of the information after propagation in GNN is higher due to the highly variable number of neighbors \cite{tailor2020degree}, it is particularly challenging to design a low-bit uniform quantization. \citet{tailor2020degree} use percentiles to empirically decide the quantization range $[\alpha,\beta]$, and a $momentum$ parameter to perform weighted average of the dynamic statistics of the tensors during training for smoothing the quantization process. We have empirically observed during experiments that low-bit quantization accuracy is sensitive to the setting of percentiles and $momentum$, which increases the difficulty of automatically obtaining accurate low-bit quantization models. 
% Fig \ref{fig_quantized_elements}, Fig \ref{separate_distribution},  Fig \ref{merge_distribution}

% Fig \ref{separate_distribution} is an example of Cora dataset \cite{mccallum2000automating} that shows the  distributions of the separate elements from the same layer in GCN.

% Low-bit quantization accuracy is sensitive to the setting of percentiles and $momentum$, which increases the difficulty of automatically obtaining accurate low-bit quantization models.
% Notes: the previous observaton
% Fig {to\_add} illustrates that different nodes from the same aggregate output tensor follow different distribution, i.e., long-tailed distribution and heavy-tailed distribution, which can be approximated as Laplacian and Gaussian distributions, respectively. In our experimental study, the nodes following the Laplacian distribution are more sensitive with a narrower quantization range, the reason is with the same quantization range, the mean overload distortion quantization (in Equation \ref{{eq:quantized_MSE}}) is larger with the long-tailed distribution, hence applying the same quantization range for them will increase the distortion.

To address these challenges, we propose a quantization approach with learnable ranges (QLR) that automatically determines the quantization range to avoid problems encountered in manually setting the percentiles and $momentum$ in low-bit quantization cases. QLR can be seen as a variant of the Learned Step Size \cite{esser2019learned}, but QLR only works for setting proper quantization range, but not 
directly learn the step size (scale) as \cite{esser2019learned}.
% Following is a distribution adaptive grouped quantization method to quantize nodes following different distributions separately.



\subsection{Quantization Error Analysis}

% \TG{This paragraph is disconnected from the previous paragraph on graph definition. Make a connection with $U$.}
For simplicity of analysis, let $U$ (e.g. $\mathbf{H^{l}}$)  represent a high-precision tensor-valued random variable with probability density function $f_U(u)$.
A tensor is commonly quantized between its maximum and minimum \emph{observed} values \citep{jacob2017gemmlowp}.
%The observed values are $U_{o}$ $\in$ $[\alpha, \beta]$, and $U$ is quantized into b-bit integer $U_q$ $\in$ $[\alpha_q, \beta_q]$, the quantization function is 
Considering observed values as $U_{o}$ $\in$ $[\alpha, \beta]$ and the corresponding $b$-bit quantized values as $U_q$ $\in$ $[\alpha_q, \beta_q]$, the quantization function is given by
\begin{equation}
Q(U, s, z) = \mathrm{clip}\Big(\lfloor\frac{U}{s}+z\rceil, \alpha_q, \beta_q\Big) = U_q
\label{eq:quantization_function}
% \mathrm{round}
\end{equation}
where $s =\frac{\beta-\alpha}{\beta_q-\alpha_q}$ is the scale, $\lfloor \cdot \rceil$ denotes the round function, 
% \TG{scale or we usually call this 'quantization factor'. Of course, we can follow the GNN quantization literature.} 
and $z=\lfloor\frac{\beta\alpha_q - \alpha\beta_q}{\beta-\alpha}\rceil$ is the zero point. The de-quantization function is as follows
% \TG{this is kind of trivial. Do we need to write this as a separate function? I would suggest writing in-line somewhere that $\hat{U} = (U_q - z)s$. This may also simplify things.}
\begin{equation}
D(U_q, s, z) =s(U_q-z)
\label{eq:dequantization_function}
\end{equation}


The range $[\alpha, \beta]$ is usually partitioned into 2$^{b}$ equal interval regions with a quantization step $\Delta = \frac{\beta - \alpha}{2^{b}}$.
If the de-quantized value is represented as $\hat{U}=(U_q- z)s$, the mean squared error (MSE) or total average distortion between $U$ and $Q(U)$ 
% \TG{check this, what you have in the equation is $U$ and $D(U_q)$} 
is given by
%Therefore, the mean sq\hat{\alpha}uared error(also called total average distortion) between $U$ and $Q(U)$ can be written as follows:
\begin{equation}
% \centering
\small
\begin{aligned}
E[(U - \hat{U})^{2}] =% \int_{-\infty}^{\infty}f(u)(u-\hat{u})^2dx \\&
&\underbrace{\int_{-\infty}^{\alpha}f_U(u)(u-\hat{\alpha})^2 du}_\text{overload} + %\\
%&
\underbrace{\int_{\beta}^{\infty}f_U(u)(u-\hat{\beta})^2du}_\text{overload} \\
+ &\underbrace{\sum_{i=0}^{2^b-1}\int_{\alpha+i\Delta}^{\alpha+(i+1)\Delta}f_U(u)(u-\hat{u})^2du}_\text{granular}
\end{aligned}
\label{eq:quantized_MSE}
\end{equation}
% \begin{equation}
% \begin{aligned}
% \int_{\alpha}^{\beta}f(u)(u-\hat{u})^2dx  \approx % \int_{-\infty}^{\infty}f(u)(u-\hat{u})^2dx \\&
%   \int_{\alpha}^{\beta}f(u)(u-\hat{u})^2dx 
% \end{aligned}
% \label{eq:quantized_MSE}
% \end{equation}
% \TG{what are $\hat{\alpha}$ and $\hat{\beta}$? don't think you have mentioned before.}

The MSE consists of three terms combining \emph{overload distortion}, $E_{ol}$, caused by the clipping operation for values of $u$ beyond $[\alpha, \beta]$, and \emph{granular distortion}, $E_{gran}$ the quantization error introduced by the quantization step $\Delta$. 
For any $U=u \in [\alpha, \beta]$, its granular distortion is in $[-\frac{\Delta}{2},\frac{\Delta}{2}]$ depending on $f_U(u)$. %the probability density distribution of the input. 
%The size of $\Delta$ is determined by $[\alpha, \beta]$ and the quantization levels 2$^b$, 
%a smaller quantization level will enlarge $\Delta$ and further increase the quantization error. 
% The larger the value of $\Delta$, the larger is the quantization error. 
Therefore, $E_{gran}$ can be reduced by setting the proper 
% \TG{optimal?}
$\Delta$ according to the distribution of $U$.



% More detailed analysis is presented in Appendix \ref{appendix_quantization_error}. 

% \begin{equation}
% \Delta = \frac{\beta - \alpha}{2^{b}}
% \label{eq:equal_intervals}
% \end{equation}
% which takes smaller percentiles but ignoring them will   since there will be more sample points be excluded for the node satisfying Gaussian distribution.

% applying the same quantization function over them will reduce the resolution of the quantization
\subsection{Oversmoothing in GNNs}

Large-scale GNNs suffer from the oversmoothing problem since adding more layers in deeper GNN architectures increase the receptive field for each node eventually creating a model that treats the nodes identically and node representations converging to indistinguishable vectors. This phenomena seriously degrades the accuracy of the overall tasks using the learned node representations. It is shown that GCNs could lose its expressive power for node classification exponentially in many practical cases \cite{oono2019GraphNeuralNetworks}.  There are some recent proposals to mitigate the oversmoothing problem \cite{liu2021elastic,rong2019dropedge,zhao2019pairnorm,liu2020towards}, including a propagation scheme based on personalized PageRank and its approximation \textbf{APPNP} \cite{klicpera2018predict}.

While deeper GNNs aim to extract more meaningful network representations, they have larger sizes which makes their deployment on constrained compute platforms like mobile devices and edge applications more challenging. This motivates the need for inference friendly compression methods that reduce the size of GNNs with efficient inference and without significant degradation in accuracy.
% Using these insights, we propose a grouped quantization approach utilizing the distribution properties of GNN components to achieve accurate compact representation with lower-bit quantizers. Specifically, we design two mechanisms for grouped quantization: layer-wise distribution-based grouping and structural similarity-based grouping.

% We observe that the quantization ranges of these elements are overlapping and the quantization steps ($\Delta$) of these quantization functions are larger which increases the quantization error.
% In the existing work for GNN quantization \cite{tailor2020degree}, independent quantization functions are applied for quantizing these elements respectively.

% We observe that the quantization ranges of these elements are overlapping and the quantization steps ($\Delta$) of these quantization functions are larger which increases the quantization error. We can take the overall distribution of these elements as a whole and find optimal partitions over the whole range to get more accurate quantization representation and decrease total error. Figure \ref{merge_distribution} shows the results when these elements are repartitioned into five sets with  equal intervals with new quantization functions applied. Fig \ref{sperateOverall_quantized_error} presents the quantization error ratios between the independent distributions and overall distribution with respect to different number of bits for quantization. We observe that using a simple partitioning,  the quantization error is reduced to one-fifth of the independent quantization in very low bitrate cases.



% \begin{figure}[tb] 
% % \centering 
% \subfigure[Independent distributions]
% {\includegraphics[height=1.3in,width=1.6in]{plots/independent_distributions_1.png} \label{separate_distribution}} 
% \hspace{-3mm}
% \subfigure[Overall distribution]{ \includegraphics[height=1.3in,width=1.6in]{plots/merge_distribution_1.png} \label{merge_distribution}} 
% \centering\caption{Distribution of the quantized elements at the same layer of GCN. 
% % \TG{These $Q_1$, $Q_2$.. has to be explained in the text or in the caption, preferrably in both places.}
% }
% \label{fig_quantized_elements}
% \end{figure}
% \begin{figure}[tb] 
% % \centering 
% \includegraphics[height=1.5in,width=2.7in]{plots/distribution_error_example.png}
% \centering\caption{The ratios of the quantization error between the independent distributions and overall distribution 
% % \TG{Please remove the background (make it white), label x and y axis, please import the figure as PDF or EPS.}
% }
% \label{sperateOverall_quantized_error}
% \end{figure}

==> plots/merge_different_k_results.tex <==
\newcommand{\realplot}[1]{
\begin{tikzpicture}
    \begin{axis}
        \addlegendimage{empty legend}\addlegendentry{Matrix #1}
        \addplot {0};
        \addplot {1};
        \addplot {2};
        \addplot {3};
    \end{axis}
\end{tikzpicture}}
    % argument #1: any options
    \newenvironment{customlegend}[1][]{%
        \begingroup
        % inits/clears the lists (which might be populated from previous
        % axes):
        \csname pgfplots@init@cleared@structures\endcsname
        \pgfplotsset{#1}%
    }{%
        % draws the legend:
        \csname pgfplots@createlegend\endcsname
        \endgroup
    }%

    % makes \addlegendimage available (typically only available within an
    % axis environment):
    \def\addlegendimage{\csname pgfplots@addlegendimage\endcsname}
\pgfplotsset{
cycle list={%
{draw=black,mark=star,solid},
{draw=black, mark=square,solid},%densely dashed}, 
{draw=black,mark=+,solid},%dashdotted}, %every mark/.append style={rotate=90},
{black,mark=o},}}
\begin{figure}[ht]
\hspace{10ex}
   \begin{tikzpicture}
        \begin{customlegend}[legend columns=4,legend style={align=left,draw=none,column sep=2ex},legend entries={Method A ,Method B ,Method C,Method D}]
        \addlegendimage{mark=star,solid,line legend}
        \addlegendimage{mark=square,solid}   
        \addlegendimage{mark=+,solid}
        \addlegendimage{mark=o}
        \end{customlegend}
     \end{tikzpicture}

\realplot{1}\realplot{2}\realplot{3}
\realplot{4}\realplot{5}\realplot{6}
\end{figure}
 

==> plots/plot_smoothness_quant_example.tex <==
\begin{figure}[tb]
\centering
% \vspace{-2mm}
\subfigure[train accuracy]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=1.2in, height=1.2in]{plots/plot_CS_smp_emp_example_train_accuracy.png}\label{train_accuracy_SMP}
%\caption{fig1}
\end{minipage}%
}% 
\subfigure[valid accuracy]{
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=1.2in, height=1.2in]{plots/plot_CS_smp_emp_example_valid_accuracy.png}\label{valid_accuracy_SMP}
%\caption{fig1}
\end{minipage}%
}% 
\subfigure[test accuracy]{
\vspace{-2mm}
\begin{minipage}[t]{0.33\linewidth}
\centering
\includegraphics[width=1.2in, height=1.2in]{plots/plot_CS_smp_emp_example_test_accuracy.png}\label{test_accuracy_SMP}
%\caption{fig1}
\end{minipage}%
}% 
\centering
\caption{Quantization performance of SMP and EMP on CS}
\label{SMP_EMP_accuracy_example}
\end{figure}

==> plots_experiment/general_accuracy_performance.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{ccccc}
\hline
Method                                                                  & Model & Cora                 & Citeseer             & Reddit-bin           \\ \hline
\multirow{3}{*}{FP32}                                                   & GCN   &                      &                      &                      \\ \cline{2-5} 
                                                                        & GAN   &                      &                      &                      \\ \cline{2-5} 
                                                                        & GIN   &                      &                      &                      \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}QAT\\ (8 bit)\end{tabular}}  & GCN   &                      &                      &                      \\ \cline{2-5} 
                                                                        & GAN   &                      &                      &                      \\ \cline{2-5} 
                                                                        & GIN   &                      &                      &                      \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}DQ\\ (8 bit)\end{tabular}}   & GCN   &                      &                      &                      \\ \cline{2-5} 
                                                                        & GAN   &                      &                      &                      \\ \cline{2-5} 
                                                                        & GIN   &                      &                      &                      \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}LQR\\ (8 bit)\end{tabular}}  & GCN   &                      &                      &                      \\ \cline{2-5} 
                                                                        & GAN   &                      &                      &                      \\ \cline{2-5} 
                                                                        & GIN   &                      &                      &                      \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}GLQR\\ (8 bit)\end{tabular}} & GCN   &                      &                      &                      \\ \cline{2-5} 
                                                                        & GAN   &                      &                      &                      \\ \cline{2-5} 
                                                                        & GIN   &                      &                      &                      \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}QAT\\ (4 bit)\end{tabular}}  & GCN   & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \cline{2-5} 
                                                                        & GAN   & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \cline{2-5} 
                                                                        & GIN   & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}DQ\\ (4 bit)\end{tabular}}   & GCN   & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \cline{2-5} 
                                                                        & GAN   & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \cline{2-5} 
                                                                        & GIN   & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}LQR\\ (4 bit)\end{tabular}}  & GCN   & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \cline{2-5} 
                                                                        & GAN   & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \cline{2-5} 
                                                                        & GIN   & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}GLQR\\ (4 bit)\end{tabular}} & GCN   & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \cline{2-5} 
                                                                        & GAN   & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \cline{2-5} 
                                                                        & GIN   & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \hline
\end{tabular}
\end{table}

==> plots_experiment/introductory_example_Table.tex <==

% \begin{table*}[tb]
% % \renewcommand\arraystretch{0.8}
%  \caption{\centering Quantization performance on Cora with the existing deep GNN solutions
% 	}
% 	\centering
% \small
%  \begin{threeparttable}
% \begin{tabular}{c|ccc|ccc}
% \toprule
%   & \multicolumn{3}{c|}{2 layer} & \multicolumn{3}{c}{10 layer} \\
%          & FP      & INT8    & INT4    & FP       & INT8    & INT4    \\
% \hline         
% DropEdge & 77.23 $\pm$ 1.58 & 78.22 \pm 1.45 & 73.73 \pm 2.94 & 76.08 \pm 2.86  & 78.90 \pm 1.46 & 39.27 \pm 1.55 \\
% PairNorm & 74.36 \pm 1.51 & 71.04 \pm 3.66 & -- -- & 71.20 \pm 2.14  & 69.3 \pm 4.60 & -- -- \\
% \hline

% \end{tabular}

% \begin{tablenotes}
%   \footnotesize
%           \item[-- --] denotes extremely low accuracy

%  \end{tablenotes}
%  \end{threeparttable}
%  \label{introductory_example_table}
% %  \vspace{-5mm}
% \end{table*}
% \vspace{-8mm}
% \begin{table}[]
% \begin{tabular}{ccccccc}
%          & \multicolumn{3}{c}{2 layer} & \multicolumn{3}{c}{10 layer} \\
%          & FP      & INT8    & INT4    & FP       & INT8    & INT4    \\
% DropEdge & 0.00 00 & 0.00 00 & 0.00 00 & 0.00 00  & 0.00 00 & 0.00 00 \\
% PairNorm & 0.00 00 & 0.00 00 & 0.00 00 & 0.00 00  & 0.00 00 & 0.00 00
% \end{tabular}
% \end{table}

% \begin{table*}[tb]
%  \caption{Classfication accuracy (\%) and model size (MB) on benchmark datasets 
% 	}
% 	\\ \textbf{(10 layers, hidden size 64)}
% 	\centering
% 	\begin{threeparttable}
% \begin{tabular}{p{1.3cm}p{1.3cm}|cc|cc|cc|cc}
% \toprule
%   \multicolumn{2}{c|}{Dataset}                 & \multicolumn{2}{c|}{Cora}  & \multicolumn{2}{c|}{Citeseer} & \multicolumn{2}{c|}{PubMed} & \multicolumn{2}{c}{Coauthor-CS} \\
% \midrule
% \multirow{4}{*}{GCN}    & FP                          & 00.00 \pm 0.00 & MB    &  00.00 \pm 0.00 & MB       &  00.00 \pm 0.00   & MB   &  00.00 \pm 0.00 & MB \\\cline{2-3} \cline{5-5} \cline{7-7} \cline{9-9}
%                           & FP^{+}   & 00.00 \pm 0.00 & MB    &  00.00 \pm 0.00 & MB       &  00.00 \pm 0.00   & MB   &  00.00 \pm 0.00 & MB \\ \cline{2-10} 
                   
%                           \hline
% \multirow{4}{*}{APPNP}    & FP                          & 00.00 \pm 0.00 & MB    &  00.00 \pm 0.00 & MB       &  00.00 \pm 0.00   & MB   &  00.00 \pm 0.00 & MB \\
%                           & FP^{+}   & 00.00 \pm 0.00 & MB    &  00.00 \pm 0.00 & MB       &  00.00 \pm 0.00   & MB   &  00.00 \pm 0.00 & MB \\
                  
%                           \hline
% \multirow{4}{*}{DropEdge} & FP                          & 00.00 \pm 0.00 & MB    &  00.00 \pm 0.00 & MB       &  00.00 \pm 0.00   & MB   &  00.00 \pm 0.00 & MB \\
%                           & FP^{+}   & 00.00 \pm 0.00 & MB    &  00.00 \pm 0.00 & MB       &  00.00 \pm 0.00   & MB   &  00.00 \pm 0.00 & MB \\
                       
%                           \hline
% \multirow{4}{*}{PairNorm} & FP                          & 00.00 \pm 0.00 & MB    &  00.00 \pm 0.00 & MB       &  00.00 \pm 0.00   & MB   &  00.00 \pm 0.00 & MB \\
%                           & FP^{+}   & 00.00 \pm 0.00 & MB    &  00.00 \pm 0.00 & MB       &  00.00 \pm 0.00   & MB   &  00.00 \pm 0.00 & MB \\
                      
%                           \hline
% \multirow{4}{*}{EMP}      & FP                          & 00.00 \pm 0.00 & MB    &  00.00 \pm 0.00 & MB       &  00.00 \pm 0.00   & MB   &  00.00 \pm 0.00 & MB \\
%                           & FP^{+}   & 00.00 \pm 0.00 & MB    &  00.00 \pm 0.00 & MB       &  00.00 \pm 0.00   & MB   &  00.00 \pm 0.00 & MB \\
                       
%                           \hline
% \multirow{4}{*}{AdMP}     & FP                          & 00.00 \pm 0.00 & 0.36MB    &  00.00 \pm 0.00 & MB       &  00.00 \pm 0.00   & MB   &  00.00 \pm 0.00 & MB \\
%                           & FP^{+}   & 00.00 \pm 0.00 & MB    &  00.00 \pm 0.00 & MB       &  00.00 \pm 0.00   & MB   &  00.00 \pm 0.00 & MB \\
                     
% \bottomrule
% \small
% \end{tabular}
%  \begin{tablenotes}
%   \footnotesize
%           \item[+] denotes that BlockMessage(BM) is integrated with the baselines.

%  \end{tablenotes}
%  \end{threeparttable}
%  \label{allbaselin_quant_performance}
% \end{table*}

		
\begin{table}[tb]
\renewcommand\arraystretch{0.9}
% \vspace{-3mm}
 \caption{\centering Quantization performance on Cora
 % with the existing deep GNN solutions
	}
% 	\\ \textbf{(10 layers, hidden size 64)}
	\centering
% 	\begin{threeparttable}
% \begin{tabular}{p{1.3cm}p{1.3cm}|cc|cc|cc|cc}
% \linespread{1.5}
 \begin{threeparttable}
 % \small
% \begin{tabular}{p{0.60cm}p{0.9cm}|c|c}
% \begin{tabular}{p{0.60cm}p{0.9cm}|c|c}
% \toprule
%  \multicolumn{2}{c|}{}
%  & {DropEdge}   & {PairNorm}  \\
% \midrule
% \small
% \centering
% \multirow{3}{*}{\rotatebox{90}{2-layer}}&  \centering FP   & 77.23 \pm 1.58  &  74.36 \pm 1.51\\

%                      & \centering  INT8 & 78.22 \pm 1.45 & 71.04 \pm 3.66 \\
%                      & \centering  INT4 & 73.73 \pm 2.94 &  — — \\
%                      \hline           
                      
% \centering
% \multirow{3}{*}{\rotatebox{90}{10-layer}} & \centering  FP   & 76.08 \pm 2.86  &  71.20 \pm 2.14\\

%                      & \centering  INT8 & 78.90 \pm 1.46 & 69.30 \pm 4.60 \\
%                      & \centering  INT4 & — —  &  — — \\
%                      \hline                         
% \end{tabular}

\begin{tabular}{c|cc|cc}
\hline
      & \multicolumn{2}{c|}{DropEdge}                & \multicolumn{2}{c}{PairNorm}                \\ \hline
layer & \multicolumn{1}{c|}{2}          & 10         & \multicolumn{1}{c|}{2}          & 10         \\ \hline
FP    & \multicolumn{1}{c|}{77.23+1.58} & 76.08+2.86 & \multicolumn{1}{c|}{73.46+1.51} & 71.20+2.14 \\
% \hline
INT8  & \multicolumn{1}{c|}{78.22+1.45} & 78.90+1.46 & \multicolumn{1}{c|}{71.04+3.66} & 69.30+4.60 \\ 
% \hline
INT4  & \multicolumn{1}{c|}{73.73+2.94} & -- --      & \multicolumn{1}{c|}{-- --}      & -- --      \\ \hline
\end{tabular}

\begin{tablenotes}
   \footnotesize
           \item[-- --] denotes extreme low accuracy
% \vspace{-5mm}
 \end{tablenotes}
 \end{threeparttable}
 \label{introductory_example_table}
 % \vspace{-5mm}
%  \vspace{-7.5mm}
\end{table}
% \vspace{-0.5mm}



==> plots_experiment/model_size_table.tex <==
% \begin{table}[tb]
% \renewcommand\arraystretch{1.15}
%  \caption{Model size (MB) on benchmark datasets 
% 	}
% % 	\\ \textbf{(10 layers, hidden size 64)}
% 	\centering
% % 	\begin{threeparttable}
% % \begin{tabular}{p{1.3cm}p{1.3cm}|cc|cc|cc|cc}
% % \linespread{1.5}
% \small
% \begin{tabular}{p{0.05cm}p{0.05cm}|c|c|c|c}
% \toprule
% \multicolumn{2}{c|}{Dataset} & \centering Cora   & \centering Citeseer & \centering PubMed & CS     \\
% \midrule
% % \small
% \multirow{3}{*}{\rotatebox{90}{\small DropEdge}} & FP   & 0.50 &  1.09 &  0.26&  1.89\\
%                     %  & FP^{+}   & 0.00 &                     & 0.00  &                      & 0.00 &                     & 0.00 &                     \\\cline{2-10}
%                      & INT8 &  0.15 &  0.29 &  0.09&  0.48\\
%                     %  & INT8^{+} & 0.00 &                     & 0.00  &                      & 0.00 &                     & 0.00 &                     \\\cline{2-10}
%                      & INT4 & 0.04 &  0.06 &  0.03&  0.08 \\
%                     %  & INT4^{+} & 0.00 &                     & 0.00  &                      & 0.00 &                     & 0.00 &                     \\

%                      \hline
% \multirow{3}{*}{\rotatebox{90}{\small PairNorm}} & FP   &  0.50 &  1.09  &  0.26&  1.89\\
%                     %  & FP^{+}   & 0.00 &                     & 0.00  &                      & 0.00 &                     & 0.00 &                     \\\cline{2-10}
%                      & INT8 &  0.16 &  0.30  &  0.10&  0.50 \\
%                     %  & INT8^{+} & 0.00 &                     & 0.00  &                      & 0.00 &                     & 0.00 &                     \\\cline{2-10}
%                      & INT4 &  0.05 &  0.07 &  0.04&  0.09\\
%                     %  & INT4^{+} & 0.00 &                     & 0.00  &                      & 0.00 &                     & 0.00 &                     \\

%                      \hline                     
% \multirow{3}{*}{\rotatebox{90}{APPNP}} & FP   & 0.62  &  1.20   & 2.30 & 5.39\\
%                     %  & FP^{+}   & 81.52 \pm 1.44 &                     & 70.31 \pm 1.53  &                      & 0.00 &                     & 0.00 &                     \\\cline{2-10}
%                      & INT8 & 0.36 & 0.48   & 2.21 & 4.09  \\
%                     %  & INT8^{+} & 0.00 &                     & 0.00  &                      & 0.00 &                     & 0.00 &                     \\\cline{2-10}
%                      & INT4 & 0.28 & 0.28  & 2.18  & 3.17 \\
%                     %  & INT4^{+} & 0.00 &                     & 0.00  &                      & 0.00 &                     & 0.00 &                     \\

%                      \hline           
                      
% \multirow{3}{*}{\rotatebox{90}{EMP/SMP}} & FP   & 0.36  &  0.93   & 0.13  & 1.75\\
%                     %  & FP^{+}   & \textbf{82.37} \pm \textbf{1.75} &                     & \textbf{71.04} \pm \textbf1.62}  &                      & \textbf{78.90} \pm \textbf{2.82} &                     & 0.00 &                     \\\cline{2-10}
%                      & INT8 & 0.10 &  0.25  & 0.05 & 0.44\\
%                     %  & INT8^{+} & 80.24 \pm 2.21 &                     & 0.00  &                      & 0.00 &                     & 0.00 &                     \\\cline{2-10}
%                      & INT4 & 0.03 & 0.04   & 0.02 & 0.07 \\
%                     %  & INT4^{+} & 0.00 &                     & 0.00  &                      & 0.00 &                     & 0.00 &                     \\

%                      \hline   
% % \multirow{3}{*}{\rotatebox{90}{SMP}} & FP   & 0.36 & 0.93  & 0.13 & 1.75\\
% %                     %  & FP^{+}   & 0.00 &                     & 0.00  &                      & 0.00 &                     & 0.00 &                     \\\cline{2-10}
% %                      & INT8 & 0.10 & 0.25  & 0.05 & 0.44 \\
% %                     %  & INT8^{+} & 0.00 &                     & 0.00  &                      & 0.00 &                     & 0.00 &                     \\\cline{2-10}
% %                      & INT4 & 0.03 & 0.04 & 0.02 & 0.07 \\
% %                     %  & INT4^{+} & 0.00 &                     & 0.00  &                      & 0.00 &                     & 0.00 &                     \\

% %                      \hline
     
                     
% \end{tabular}
% % \begin{tablenotes}
% %   \footnotesize
% %           \item[+] denotes that BlockMessage(BM) is integrated with the baselines.

% %  \end{tablenotes}
% %  \end{threeparttable}
%  \label{allbaselin_modelsize}
% \end{table}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[tb]
\renewcommand\arraystretch{0.9}
 \caption{Model size (MB) on benchmark datasets 
	}
 \small
% \begin{tabular}{cc|c|c|c|c}
% \hline
% \multicolumn{2}{c|}{Model}                          & DropEdge & PairNorm & APPNP & EMP/SMP \\ \hline
% \multicolumn{1}{c|}{\multirow{4}{*}{\rotatebox{90}{Cora}}}     & FP   & 0.50     & 0.50     & 0.36  & 0.36    \\ 
% \multicolumn{1}{c|}{}                          & INT8 &     0.15     &    0.16      &   0.10    &    0.10     \\ 
% \multicolumn{1}{c|}{}                          & INT4 &     0.09     &    0.10      &   0.05    &   0.06      \\ 
% \multicolumn{1}{c|}{}                          & INT2 &          0.06 &     0.07     &   0.03    &    0.04     \\ \hline
% \multicolumn{1}{c|}{\multirow{4}{*}{\rotatebox{90}{\centering \small CiteSeer}}} & FP   &        1.09  &    1.09      &   0.93    &   0.93      \\ 
% \multicolumn{1}{c|}{}                          & INT8 &    0.29      &    0.30      &   0.24    &    0.25     \\  
% \multicolumn{1}{c|}{}                          & INT4 &     0.16     &     0.17     &    0.13   &    0.13     \\ 
% \multicolumn{1}{c|}{}                          & INT2 &          0.09 &     0.10     &    0.07   &     0.07    \\ \hline
% \multicolumn{1}{c|}{\multirow{4}{*}{\rotatebox{90}{\centering \small PubMed}}}   & FP   &       0.26   &    0.26      &   0.13    &   0.13      \\ 
% \multicolumn{1}{c|}{}                          & INT8 &    0.09      &     0.10     &   0.04    &    0.05     \\ 
% \multicolumn{1}{c|}{}                          & INT4 &      0.06    &    0.07      &  0.03     &     0.03    \\ 
% \multicolumn{1}{c|}{}                          & INT2 &          0.04 &     0.05     &    0.02   &    0.02     \\ \hline
% \multicolumn{1}{c|}{\multirow{4}{*}{\rotatebox{90}{CS}}}       & FP   &      1.89    &     1.89     &   1.75    &  1.75       \\ 
% \multicolumn{1}{c|}{}                          & INT8 &     0.48     &    0.50      &   0.44    &    0.44     \\ 
% \multicolumn{1}{c|}{}                          & INT4 &     0.25     &    0.27      &   0.22    &     0.23    \\ 
% \multicolumn{1}{c|}{}                          & INT2 &          0.14 &    0.15      &    0.12   &    0.12     \\ \hline
% \end{tabular}
\begin{tabular}{c|c|c|c|c}
\hline
     & Cora & CiteSeer & PubMed & CS   \\ \hline
FP   & 0.36 & 0.93     & 0.13   & 1.75 \\ 
INT8 & 0.10 & 0.25     & 0.05   & 0.44 \\ 
INT4 & 0.06 & 0.13     & 0.03   & 0.23 \\ 
INT2 & 0.04 & 0.07     & 0.02   & 0.12 \\ \hline
\end{tabular}
\label{allbaselin_modelsize}
\vspace{-1mm}
\end{table}

==> plots_experiment/performance_with_different_K.tex <==
\textbf{A Figure: The performance with different number of $K$ including 4-bit,8-bit and FP.}

\textbf{A Figure: The performance of DropEdge and BlockMessage with different ratio of edges get dropped/blocked}
